Model-Invariant State Abstractions for Model-Based Reinforcement Learning

Accuracy and generalization of dynamics models is key to the success of model-based reinforcement learning (MBRL). As the complexity of tasks increases, so does the sample inefficiency of learning accurate dynamics models. However, many complex tasks also exhibit sparsity in the dynamics, i.e., actions have only a local effect on the system dynamics. In this paper, we exploit this property with a causal invariance perspective in the single-task setting, introducing a new type of state abstraction called \textit{model-invariance}. Unlike previous forms of state abstractions, a model-invariance state abstraction leverages causal sparsity over state variables. This allows for compositional generalization to unseen states, something that non-factored forms of state abstractions cannot do. We prove that an optimal policy can be learned over this model-invariance state abstraction and show improved generalization in a simple toy domain. Next, we propose a practical method to approximately learn a model-invariant representation for complex domains and validate our approach by showing improved modelling performance over standard maximum likelihood approaches on challenging tasks, such as the MuJoCo-based Humanoid. Finally, within the MBRL setting we show strong performance gains with respect to sample efficiency across a host of other continuous control tasks.

==> Sections/DeepExps.tex <==
Contrastive Predictive Coding (CPC) has been used as an unsupervised learning technique, where data augmentations are used with an instance classification task. For self-supervised prediction, the two main components therefore are: 1) creating a refinement task, i.e. instance classification (b/w positive and negative samples from the data augmentation) and 2) data augmentation to create data for the classification task. This sort of a pipeline is usually attached to the actual task in hand, be it supervised prediction or RL. 

The ReLIC architecture views the data augmentations as an interventional scheme to gather data and the instance classification task as a refinement of the actual classification task in hand, which we don't know (if it's a prediction task, then we use this classification task as an auxiliary objective for the actual supervised prediction or RL task). With that analogy in mind, the data augmentations correspond to the data from different environments (in the invariance sense) and the instance classification task aims at distinguishing between an interventional data sample being legit or not. 

CURL uses a instance classification task, which is a refinement of the overall image classification task. However, for a model based learner, the refinement should be a next state prediction task. Or, in other words, that state, action, next state classification task.

When one intervenes, we see slightly different data and our task is to make sure that it's coming from the same label. Similarly, when we see multiple state, action, next state samples when we intervene, our task is to make sure that the tuple is coming from the same label. Here the label would just be if it's coming from the true dynamics model or not. The next important question is how to generate negative samples. This will be tied to the way we augment data/intervention scheme. Still not sure how the factorization comes into picture naturally. 

==> Sections/Introduction.tex <==
\section{Introduction}

Model Learning in reinforcement learning (RL) has always been considered as an attractive tool in improving the sample efficiency as well as the final performance of the learnt policies. So much so that a sub-branch of RL research has emerged from it, a.k.a model-based RL (MBRL). At its core, model-based RL talks about learning a model of the environment, and then using samples from it to either 1) fully plan, 2) to augment the data used by a completely model-free solver, or 3) to be used as an auxiliary task while training. However, learning the model, just as any other supervised learning problem, suffers from the issue of distributional shift, i.e. the data we train on is not necessarily the data we test on. This issue is worsened in RL as even a small change in the current policy can lead to visiting completely unexplored parts of the state space, and thus the learnt model predicting arbitrarily inaccurate estimates. Various workarounds exist for this issue, including coupling the model and policy learning processes, however these only manage to mitigate it to a certain extent. In this context, we ask the question, \emph{is it possible to better structure and process the data used by model learners in order to improve their ability to  generalize to unseen parts of the state space?} 

The model (more specifically, the transition dynamics) learning problem in RL is simple to pose--- we wish to learn to predict the next state given the current state and action using data collected from the agent's experience. In essence, this is a supervised learning problem, \textit{if} the training and testing policy is always learnt from a fixed state distribution (train and test distributions are same). As we know, this is not true in RL since a small change in the policy can lead to an arbitrarily large change in the state distribution. In this paper, we look to the principle of invariance to resolve this issue. For a general supervised learning prediction problem, the principle of invariance w.r.t. a set of features (observations in RL) dictates that we should aim to build representations that comprise \textit{only} those features which are consistently necessary for predicting the target variable of interest, across the combined set of all training and all testing environments. The rationale being that such features are consistent to the learning problem in hand and thus a predictor built over such features generalizes well over all environments. For the purposes of this paper, the prediction problem corresponds to learning a model of a Contextual Decision Process (CDP) while each environment corresponds to the state distribution induced by a fixed single policy over the CDP. Building on this framework, we answer the above raised question in the affirmative, by learning an invariant model of the CDP. Such a model generalizes well on state distributions induced by a policy reasonably distinct from the ones used while learning it.


To capture this notion of invariance, we propose a new kind of state abstraction, called model invariance. Model invariance has the similar in flavour to model irrelevance but applies to individual dimensions of the observation instead of the full observation as a whole. We show that a representation which only uses the causal parents of each observation dimension follows this definition of model invariance. Furthermore, we can learn a model of the CDP given such an abstraction, and show that planning using this model is optimal, given certain assumptions on the exploration. Finally, we perform a simple proof experiment in the batch setting to show that such a model learning approach leads to better generalization in unseen parts of the state space. Overall, we introduce a theoretically grounded method which improves the performance of MBRL methods in general, by learning a more accurate model of the MDP.

==> Sections/Prelimanaries.tex <==
\section{Preliminaries}

We first discuss the setup of the paper, which is followed by describing the relevant prior frameworks we use and build upon. This includes model-based RL, invariant causal prediction and state abstractions. 

\subsection{Setup}
In this paper, we assume that the agent's interaction with the environment is modeled as a discrete time $\gamma$-discounted Contextual Decision Process (CDP), a term recently proposed by \cite{krishnamurthy2016pac} to broadly model sequential decision processes which require the policy to be based on rich features (context). Particularly, a CDP is denoted by $\mathcal{M}=(\mathcal{X}, \mathcal{A},P,R,\gamma,\mu)$, where $\mathcal{X} \subseteq \mathbb{R}^{d}$ and $\mathcal{A}$ are the state and action spaces; $P \equiv P(x'|x,a)$ is the transition kernel; $R \equiv r(x,a)$ is the reward function with the maximum value of $R_{\text{max}}$; $\gamma\in(0,1)$ is the discount factor; and $\mu$ is the initial state distribution. CDPs generalize MDPs, in that they allow us to consider various other models such as POMDPS and PSRs besides regular MDPs. Let $\pi: \mathcal{X}\rightarrow \Delta_{\mathcal{A}}$ be a stationary Markovian policy, where $\Delta_{\mathcal{A}}$ is the set of probability distributions on $\mathcal{A}$. The discounted frequency of visiting a state $s$ by following a policy $\pi$ is defined as $\rho_\pi(x)\equiv (1-\gamma) \mathbb{E}[\sum_{t\geq 0}\gamma^t \mathbb I \{x_t=x\}\mid \mu, \pi]$. The value function of a policy $\pi$ at a context $x\in\mathcal{X}$ is defined as $V^\pi(x) \equiv \mathbb{E}[\sum_{t\geq 0}\gamma^tr(x_t,a_t)|x_0=x, \pi]$. Similarly, the action-value function of $\pi$ is defined as $Q^{\pi}(x,a) = \mathbb{E}[\sum_{t\geq 0}\gamma^tr(x_t,a_t)|x_0=x,a_0=a,\pi]$. Note that the CDP definition also assumes the there exists a set of latent states $\mathcal{S}$, finite in number, which we do not have access to. If we pose further structural assumptions, such as that of a Block MDP, then the notion of $S$ becomes more apparent. 

There are two important cases we can consider with CDPs. Let's explore these with examples:

1. Large state space, a.k.a full state input: Consider the example of the proprioceptive states of MuJoCo as $\mathcal{X}$. In this case, $\mathcal{X}$ is not a rich observation, but is an arbitrarily large (but mostly finite) set of states. There is very less irrelevant information present in such a case. In this case, the latent states $\mathcal{S}$ correspond to some coarser abstraction of the given full state, which can still lead to optimal learning. 

2. Rich observation a.k.a. image based input: In this case, denote by $\mathcal{\bar{X}}$ the set of images, for example, each being a front view of the MuJoCo based robot. There could be a lot of irrelevant information present in this case such as the background pixels. Nevertheless, the latent state set $\mathcal{S}$ is still the same as in the previous case, which is some coarse representation of the true MuJoCo state $\mathcal{X}$, which itself is hidden in the image based input. Therefore, our task here is even more tedious, in that we first have to extract the true state of the robot from the image (eqv. to what we were given in case 1) and then learn this coarser representation. Also note that, for us to consider case 2 as tractable, at least theoretically, we would have to assume a block MDP like structure, since otherwise having access to just the observations can lead to a POMDP setting. 

For both cases, we assume that the transition dynamics over the full state are factorized. More formally:

\begin{assumption} (Transition Factorization)
For given full state vectors $x, x^{\prime} \in \mathcal{X}$, action $a \in \mathcal{A}$, and $x_i$ denoting the $i^{\text{th}}$ dimension of state $x$ we have
\begin{equation*}
    P(x^{\prime} | x, a) = \prod_{i} P(x^{\prime}_{i} | x, a)
\end{equation*}
\end{assumption}

Note that this is a much less strict assumption than assuming factored MDPs \citep{kearns1999efficient, guestrin2001max}.

\begin{comment}
This paper, theoretically, will assume the abstraction given (oracle abstraction assumption), and the exploration problem of not much concern (concentrability assumption). The invariance part relates the significance of such an abstraction to a causal representation, in the linear case. In the nonlinear case, we can only hope that something similar is happening. Nevertheless, this has nothing to do with the theoretical results, as they assume the abstraction is already given. 

Having a bisimulation is equivalent to assuming realizabiltity and completeness, if we want to follow a value/policy based analysis/algorithm. In the model based algorithm, assuming bisimulation is enough. In our case, we are not exactly a bisimulation. But we can show that a similar sort of bound holds for our abstraction. To that end, we would need another assumption similar to a low bellman rank or something similar, which ensures that the difference in the abstraction is bounded for each dimension. 
\end{comment}


\subsection{Model-based Reinforcement Learning}
\amy{cover the methods we'll use to evaluate the causally invariant model here, e.g. MBPO, MPC}
Model-based reinforcement learning typically involves learning a dynamics model of the environment by fitting it using a maximum-likelihood estimate of the trajectory-based data collected by running some exploratory policy. Such a learned model is then used to plan for the optimal policy using techniques such as model predictive control or MPC. In the offline RL setting, where we only have access to the data collected by multiple policies, recent techniques build on the idea of pessimism (regularizing the original problem based on how confident the agent is about the learned model) and have resulted in better sample complexity over model-free methods on benchmark domains \citep{janner2019trust, kidambi2020morel, yu2020mopo}. 

\subsection{Invariant Causal Prediction}
Invariant causal prediction (ICP) \citep{peters2015causal} considers learning an invariant representation w.r.t. spurious correlations that arise due to noise in the underlying causal model \manan{define 'casual model'} that describes a given system. The key idea is that across different environments, the response variable $Y$ remains the same given the variables $X_i$ that directly cause the response variable, i.e. its parents $\textbf{PA(Y)}$. This is true under the assumption that:

\begin{itemize}
    \item There are no interventions on $Y$ itself.
    \item There exists a model which remains invariant under certain interventions/across different environmental settings, i.e. identifiability.
\end{itemize}
\amy{How does the additional requirement of an intervention per variable (other  than $Y$) translate here?}
For our purposes, we are interested in the causal diagram $(x_t, a_t) \rightarrow x_{t+1}$. The interventions in this case are with respect to the actions, and the causality is temporal in nature. Now we can naively call an environment in this case as one $(x, a, x^\prime)$ tuple. However, if the action distribution, i.e. the policy remains the same across multiple time-steps, then we essentially generate a trajectory involving the causal variables $(x, a, x^\prime)$. This data set can constitute one environment. When the policy is changed, (in other words we are intervening on the system through the policy actions), a new environment is generated. This gives us a pool of multiple environments, each consisting of a set of causal variables observed under an approximately restricted intervention scheme \manan{vague, clarify!}. In contrast, current methods of learning dynamics models in RL include mixing experience from multiple policies and then learning a mapping from $x, a$ to $x^{\prime}$. 


%Linking back to the IRM work, this can be termed as an ERM or robust representation over $s, a$ and not an invariant one. Note that the original IRM/ICP work talks about learning the direct casual set for a scalar response variable. Thus, the state prediction case is just a multi variable setting where we are interested in choosing the right representation for predicting each component of the next state. 


Note that the block MDP setting used in \cite{zhang2020invariant} assumes that there are high dimensional observations and hidden states present for a given MDP and that there exists an emission function $q_e$ which maps the hidden state $s$ to the observation $x$. The response variable here is the reward and the interventions are over the observations. The hidden state variables relating to the block MDP definition are thus the invariant set of variable components of the observations, which as it turns out, are the hidden state variables. This setting differs with the contents of this paper in two key aspects: \textbf{1)} we do not include the block MDP assumption and more importantly, \textbf{2)} we consider the causal relationship in the transition model, as opposed to the one between the state and reward.

\subsection{State Abstractions}
State abstractions allow us to condense potentially many states into a single abstract state, thus simplifying the learning problem which then makes use of the (much smaller set of) abstract states instead of the original states \citep{bertsekas1988adaptive}. In essence, any function approximation scheme can act as an abstraction, since it attempts to group similar states together. Therefore, it is worth exploring the properties of a representation learning scheme as a state abstraction. In the rest of the paper, we build our theory based on this connection. 

Here, we are interested in a specific kind of state abstraction called model irrelevance state abstraction or bisimulation \citep{even2003approximate, ravindran2004algebraic, li2009unifying}. Particularly, we say an abstraction $\phi$ is model irrelevant if for any $x^1$, $x^2 \in \mathcal{X}$, $\bar{x} \in \phi(\mathcal{X})$, $a \in \mathcal{A}$ where $\phi(x^{1}) = \phi(x^{2})$,

\begin{align*}
    &R(x^{1}, a) = R(x^{2}, a), 
    &\sum_{x^{\prime} \in \phi^{-1}(\bar{x})} P(x^{\prime} | x^{1}, a) = \sum_{x^{\prime} \in \phi^{-1}(\bar{x})} P(x^{\prime} | x^{2}, a)
\end{align*}

Since an exact equivalence is not practical, prior work deals with approximate variants through the notion of $\epsilon$ closeness \citep{jiang2018notes}.

==> Sections/RelatedWork.tex <==
\section{Related Work}

Planning based on structural assumptions on the underlying MDP have been explored in much detail before \citep{boutilier1999decision}. The most closely related setting is of factored MDPs. Learning based approaches that build on the factored MDP assumption have predominantly also assumed a known graph structure for the transition factorization \citep{kearns1999efficient, strehl2007efficient, osband2014near}.

On the theory side, most prior works on factored MDPs assume the finite state space setting, where the number of states can be exponential to the number of state variables \citep{kearns1999efficient, strehl2007efficient}. We instead discuss the rich observation setting, which requires us to talk about optimality results when abstractions are applied. 

On the algorithmic side, there have been only a few works that discuss learning the graph or DBN structure alongside the factored MDP assumption \citep{hallak2015off}. We differ from these in that we only learn the partial graph structure, i.e. only the direct parents of each state variable. Moreover, we achieve this using the invariance principle, which has not been explored in prior work, to the best of our knowledge. The primary reason for adopting the invariance principle is that it naturally allows us to work in the multiple environment setting, where an environment is characterized by the different state distributions induced by different policies during training. This is an important distinction from the supervised learning setting, a setting where other graph structure learning methods have been shown to work well. There is little reason to believe that such approaches extend to the RL case as well, particularly because the data distribution is not fixed in general in RL.

There has been quite a lot of recent work around the newly proposed CDP setting \citep{krishnamurthy2016pac, sun2019model, misra2020kinematic}. In that sense, our work has overlapping ideas with model based learning in CDPs \citep{misra2020kinematic} and learning efficient abstractions over them \citep{sun2019model}. Besides the more algorithmic and empirically focused nature of this work, there remain several considerable distinctions. First, we focus on abstraction based learning, whereas \cite{sun2019model} rely on the concept of \textit{witness misfit} to learn over the original CDP states. Second, we are focused on the learning abstract states that are a coarser representation of the true full state of the CDP, whereas \cite{misra2020kinematic} deal with the case where the abstract states correspond to the full state/latent states of the MDP. In that sense, the framework adopted here is a blend of that presented in these two works. Ideally, we would like to show that the class of problems where the number of model invariant abstract states is low, have a low \textit{witness rank} as well. 

\begin{comment}

1. Distinction b/w rich observation and large state spaces. Former can assume some latent structure but the latter probably can't. Also, latter might be large because of continuous domains. 

2. Clear distinction between assuming a factored state space (which KS do) and a factored transition distribution (which we do). KS show optimal bounds for when the state space is factored and can be large. In both rich observation and large state spaces, we are different because we build on abstraction theory based on transition factorization assumption, whereas KS only use the large state spaces setting and assume it to be factored (they basically say, if there is a factored mdp, then it would have exponentially many states. We ask the upside down question instead) . Question is how does this difference translate in both of our theoretical results?  

3. What does the transition factorization assumption translate to in both of the above settings? What are its practical implications?

4. Can we remove the concentrability assumption and bring in something like a policy cover, similar to HOMER?

5. Compare with Sun et al. as well. How does all this relate to low witness rank? Maybe points to answering 2.

The factored state space assumption only helps in removing the exponential dependence of the number of states with the number of variables/dimensions. However, we still require abstraction theory results since each variable can take infinite values in the rich observations setting. This is where we are different from KS. Worth asking question here is: what's the difference between a factored MDP assumption vs a factored transition assumption. 

The 'large state space' basically refers to having full state information but the state space being infinite. The 'rich observation' refers to a partially observable environment. I am not sure how this relates exactly to the CDP definition. Let's clarify this (based on the ICP block MDP paper) because we might be able to consider interesting connections with Sun et al. then. 

On the learning of DBNs, I think the theory there borrows from supervised learning, thus assuming that the data distribution being learnt from does not change. However, we know that this is not true in RL as when the policy changes, the data distribution changes too. This sort of multi-environment setting is precisely where ICP tries to take the upper hand. Therefore, combining the invariance principle for learning the structure of the DBN is a more suited approach, one that has not been tried before. Moreover, we are dealing with the infinite states case, therefore the abstraction results remain important as well. 

\end{comment}

